Spatial Statistical Models: an overview under the Bayesian Approach

Spatial documentation is exponentially increasing given the availability of Big IoT Data, enabled by the devices miniaturization and data storage capacity. Bayesian spatial statistics is a useful statistical tool to determine the dependence structure and hidden patterns over space through prior knowledge and data likelihood. Nevertheless, this modeling class is not well explored as the classification and regression machine learning models given their simplicity and often weak (data) independence supposition. In this manner, this systematic review aimed to unravel the main models presented in the literature in the past 20 years, identify gaps, and research opportunities. Elements such as random fields, spatial domains, prior specification, covariance function, and numerical approximations were discussed. This work explored the two subclasses of spatial smoothing global and local.

==> h5tg93k20to.tex <==
\subsection{LaTeX and Mathematical notation}
\label{sec:latex}
You can also include LaTeX code in your documents. Here is a simple inline equation $e^{i\pi}=-1$ and here's a longer equation, numbered:

\begin{equation}
\label{eqn:some}
\int_0^{+\infty}e^{-x^2}dx=\frac{\sqrt{\pi}}{2}
\end{equation}

==> header.tex <==
% Add any additional LaTeX packages and macros here
\usepackage{siunitx}

%---

\iflatexml
% Add any LateXML specific commands here

%---

\else
% The commands below will only change the exported PDF. Edit or remove as needed

\paperfield{Field of the paper}
\abbrevs{ABC, a black cat; DEF, doesn't ever fret; GHI, goes home immediately.}
\corraddress{Author One PhD, Department, Institution, City, State or Province, Postal Code, Country}
\corremail{correspondingauthor@email.com}
\presentadd{Department, Institution, City, State or Province, Postal Code, Country}
\fundinginfo{Funder One, Funder One Department, Grant/Award Number: 123456, 123457 and 123458; Funder Two, Funder Two Department, Grant/Award Number: 123459}
\fi

%---
